SeePrivacy: Automated Contextual Privacy Policy Generation for Mobile Applications

Privacy policies have become the most critical approach to safeguarding individuals' privacy and digital security. To enhance their presentation and readability, researchers propose the concept of contextual privacy policies (CPPs), aiming to fragment policies into shorter snippets and display them only in corresponding contexts. In this paper, we propose a novel multi-modal framework, namely SeePrivacy, designed to automatically generate contextual privacy policies for mobile apps. Our method synergistically combines mobile GUI understanding and privacy policy document analysis, yielding an impressive overall 83.6% coverage rate for privacy-related context detection and an accuracy of 0.92 in extracting corresponding policy segments. Remarkably, 96% of the retrieved policy segments can be correctly matched with their contexts. The user study shows SeePrivacy demonstrates excellent functionality and usability (4.5/5). Specifically, participants exhibit a greater willingness to read CPPs (4.1/5) compared to original privacy policies (2/5). Our solution effectively assists users in comprehending privacy notices, and this research establishes a solid foundation for further advancements and exploration.

==> DataAvailability.tex <==
\section{Data Availability}
Our dataset and codes are available at \url{https://github.com/Cpp4App/Cpp4App}.


==> Tables/interested_class.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llrrr}
\toprule
\textbf{RICO-icon Class} & \textbf{Data type} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} \\
\midrule
Call  & Phone & 0.70 & 1.00 & 0.70 \\
Email  & Email & 0.74 & 0.68 & 0.81 \\
Avatar  & Profile & 0.85 & 0.82 & 0.89 \\
Follow & Contacts & 0.90 & 0.82 & 1.00 \\
Group  & Contacts &  0.67 & 0.73 & 0.62   \\
Location  & Location & 0.89 & 0.86 & 0.92 \\
Location crosshair & Location & 0.72 & 0.63 & 0.83 \\
Photo & Photos & 0.87 & 0.89 & 0.85 \\
Wallpaper  & Photos & 0.87 & 0.82  & 0.93 \\
Videocam  & Photos &  0.91 & 0.83 & 1.00 \\
Microphone  & Voices & 0.96 & 0.93  & 1.00   \\
Cart &  Financial Info & 0.81 & 0.75   &   0.88   \\
Facebook  & Social media & 0.83 & 0.75 & 0.92  \\
Twitter  & Social media & 0.90  & 0.95 & 0.86 \\
\midrule
\textbf{Average} & &  0.82 & 0.83 & 0.85  \\
\bottomrule
\end{tabular}
\caption{Performance of ours network on context-related RICO-icon classes.}
\label{tab_classification_perclass}
\end{table}

% Old model
% Call  & Phone & 0.70 & 1.00 & 0.70 \\
% Email  & Email & 0.49 & 0.55 & 0.81 \\
% Avatar  & Profile & 0.70 & 0.88 & 0.77 \\
% Follow & Contacts & 0.50 & 0.56 & 0.83 \\
% Group  & Contacts & 0.58 & 0.88 & 0.64 \\
% Location  & Location & 0.59 & 0.91 & 0.63 \\
% Location crosshair & Location & 0.77 & 0.89 & 0.86 \\
% Photo & Photos & 0.73 & 0.83 & 0.86 \\
% Wallpaper  & Photos & 0.61 & 0.70 & 0.83 \\
% Videocam  & Photos & 0.71 & 0.83 & 0.83 \\
% Microphone  & Voices & 0.93 & 0.96 & 0.96 \\
% Facebook  & Social media & 0.68 & 0.85 & 0.77 \\
% Twitter  & Social media & 0.95 & 0.95 & 1.00 \\
% \midrule
% \textbf{Average} & & 0.69 & 0.81 & 0.81    \\
% Location crosshair & Location & 0.774 & 0.889 & 0.857 \\
% Photo & Photos & 0.731 & 0.826 & 0.864 \\
% Facebook  & Social media & 0.680 & 0.850 & 0.773 \\
% Microphone  & Voices & 0.931 & 0.964 & 0.964 \\
% Email  & Email & 0.486 & 0.548 & 0.810 \\
% Twitter  & Social media & 0.952 & 0.952 & 1.000 \\
% Location  & Location & 0.594 & 0.905 & 0.633 \\
% Call  & Phone & 0.696 & 1.000 & 0.696 \\
% Wallpaper  & Photos & 0.609 & 0.700 & 0.824 \\
% Follow & Contacts & 0.500 & 0.560 & 0.824 \\
% Group  & Contacts & 0.583 & 0.875 & 0.636 \\
% Avatar  & Profile & 0.698 & 0.88 & 0.772 \\
% Videocam  & Photos & 0.714 & 0.833 & 0.833 \\
% Play  & Example 14 & 0.800 & 0.897 & 0.881 \\


==> Tables/keywords_icons_match.tex <==
\begin{figure*}[htbp]
\centering
\begin{spacing}{} 
\setlength\tabcolsep{1pt} 
\begin{tabular}{ccc}
             Privacy-related information & Icon   \\
\hline
Camera & \begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera1.png}}\end{minipage} &     
		\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera2.png}}
	\end{minipage}               \\ \\
Camera &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera3.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera4.png}}
	\end{minipage}              \\ \\
 Email &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/email1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/email2.png}}
	\end{minipage}              \\ \\
 Location &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/location1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/location2.png}}
	\end{minipage}              \\ \\
Contacts &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts2.png}}
	\end{minipage}              \\ \\
 Contacts &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts3.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts4.png}}
	\end{minipage}              \\ \\
 Financial information &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/financial1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/finantial2.png}}
	\end{minipage}              \\ \\
 Microphone &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/microphone1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/microphone2.png}}
	\end{minipage}              \\ \\
 Personal identifier &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/profile1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/profile2.png}}
	\end{minipage}              \\ \\
 Phone &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/phone1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/phone2.png}}
	\end{minipage}              \\ \\
 Social Media &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/social1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/social2.png}}
	\end{minipage}              \\ \\

\end{tabular}
\end{spacing}

\vspace{2em}
\label{tab_match}
\caption{Matching of CPP-related privacy keywords and icons.}
\end{figure*}

==> Tables/keywords_summary.tex <==
\begin{table*}[!t]
  \caption{Important data types exist in the literature.}
  \vspace{-5pt}
  \label{tab_survey}
  \centering
  \resizebox{.9\textwidth}{!}{%
  \begin{tabular}{l|cccccc|cccccc}
    \hline
    \rowcolor{lightgray!15}
    &                                                                                        \multicolumn{6}{c|}{Basic Personal Identifiable Information}                                                                       & \multicolumn{6}{c}{Other Personal Information}                                                                                     \\ 
    \hline
    \rowcolor{lightgray!85}
    &Name & Birthday & Address & Phone & Email &Profile
    & Contacts & Location & Photos & Voices & Financial Info 
    & Social Media \\
    \hline
    
    \rowcolor{lightgray!50}
    \textbf{Administration}
    & & & & & & & & & & & &\\
    \rowcolor{lightgray!15}
    GDPR~\cite{GDPR} 
    & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE
    & \Circle &\Circle &\Circle &\Circle &\Circle &\Circle 
    \\
    \rowcolor{lightgray!15}
    CCPA~\cite{CCPA} 
    & \CIRCLE &\Circle &\Circle &\Circle &\CIRCLE &\CIRCLE
    & \Circle &\CIRCLE &\Circle &\Circle &\CIRCLE &\Circle 
     \\
    \rowcolor{lightgray!15}
    CalOPPA~\cite{CalOPPA} 
    & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\Circle
    & \Circle &\CIRCLE &\Circle &\Circle &\CIRCLE&\CIRCLE 
    \\
    \rowcolor{lightgray!15}
    COPPA~\cite{COPPA} 
    & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE
    & \Circle &\CIRCLE &\CIRCLE &\CIRCLE &\Circle&\Circle 
    \\
    
    \rowcolor{lightgray!15}
    APP~\cite{APP} 
    &\CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE
    &\Circle &\CIRCLE &\CIRCLE &\Circle &\CIRCLE &\Circle
    \\
    
    \rowcolor{lightgray!50}
    \textbf{Industry}
    & & & & & &  & & & & & & \\
    \rowcolor{lightgray!15}
    Google~\cite{googledatasafety} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    \\
    % Google contains the MAC address
    \rowcolor{lightgray!15}
    Apple~\cite{appleprivacy} 
    & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Huawei~\cite{Huaweiprivacy} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
    \\
    \rowcolor{lightgray!15}
    Amazon~\cite{Amazonprivacy} 
    & \Circle & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    \\
    
    \rowcolor{lightgray!50}
    \textbf{Academia} &&&&&& &&&&&&\\
    \rowcolor{lightgray!15}
    Yu et al.~\cite{yu2015autoppg} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    \\
    \rowcolor{lightgray!15}
    Wilson et al.~\cite{wilson2016creation} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Harkous et al.~\cite{harkous2018polisis} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Kaur et al.~\cite{kaur2018comprehensive} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE  & \Circle
    \\
    \rowcolor{lightgray!15}
    Yu et al.~\cite{yu2018enhancing}
    & \Circle & \Circle & \Circle & \Circle & \Circle & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    \\
    \rowcolor{lightgray!15}
    Zimmeck et al.~\cite{zimmeck2019maps} 
    & \Circle & \Circle & \Circle & \CIRCLE & \CIRCLE & \CIRCLE
    & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Zhang et al.~\cite{zhang2020does} 
    & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle
    & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle
    \\
    \rowcolor{lightgray!15}
    Sun and Xue~\cite{sun2020quality} 
    & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle
    & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle
    \\
   
    \rowcolor{lightgray!15}
    Li et al.~\cite{li2021developers} 
    & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    \\
    % \rowcolor{lightgray!15}
    % Only focus on analytics libraries rather than apps
    % Caputo et al.~\cite{caputo2021you} 
    % & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
    % & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    % & \CIRCLE & \Circle\\

    \rowcolor{lightgray!15}
    Zimmeck et al.~\cite{zimmeck2021privacyflash} 
    & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle
    & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \CIRCLE
    \\
     
    \rowcolor{lightgray!15}
    Xie et al.~\cite{xie2022scrutinizing} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle
    \\
  \hline
\end{tabular}
}%
\vspace{-14pt}
\end{table*}


% \begin{table*}[!t]
%   \caption{Important data types existence in literature.}
  
%   \label{tab_survey}
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|ccccc|cccccc|cc}
%     \hline
%     \rowcolor{lightgray!15}
%     &                                                                                        \multicolumn{5}{c|}{Basic Personal Identifiable Information}                                                                       & \multicolumn{6}{c|}{Other Personal Information}                                                                                     & \multicolumn{2}{l}{Online Identifiers} \\ 
%     \hline
%     \rowcolor{lightgray!85}
%     &Name & Birthday & Address & Phone & Email 
%     & Contacts & Location & Photos & Voices & Financial Info 
%     & Social Media &IP & Cookies \\
%     \hline
    
%     \rowcolor{lightgray!50}
%     \textbf{Administration}
%     & & & & & & & & & & & & &\\
%     \rowcolor{lightgray!15}
%     GDPR~\cite{GDPR} 
%     & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     & \Circle &\Circle &\Circle &\Circle &\Circle &\Circle 
%     & \CIRCLE &\CIRCLE\\
%     \rowcolor{lightgray!15}
%     CCPA~\cite{CCPA} 
%     & \CIRCLE &\Circle &\Circle &\Circle &\CIRCLE 
%     & \Circle &\CIRCLE &\Circle &\Circle &\CIRCLE &\Circle 
%     & \Circle &\Circle \\
%     \rowcolor{lightgray!15}
%     CalOPPA~\cite{CalOPPA} 
%     & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     & \Circle &\Circle &\Circle &\Circle &\Circle&\Circle 
%     & \CIRCLE &\CIRCLE\\
%     \rowcolor{lightgray!15}
%     COPPA~\cite{COPPA} 
%     & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     & \Circle &\CIRCLE &\CIRCLE &\CIRCLE &\Circle&\Circle 
%     & \CIRCLE &\CIRCLE\\
    
%     \rowcolor{lightgray!15}
%     APP~\cite{APP} 
%     &\CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     &\Circle &\CIRCLE &\CIRCLE &\Circle &\CIRCLE &\Circle
%     &\CIRCLE &\Circle\\
    
%     \rowcolor{lightgray!50}
%     \textbf{Industry}
%     & & & & & & & & & & & & &\\
%     \rowcolor{lightgray!15}
%     Google~\cite{googledatasafety} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \Circle & \Circle\\
%     % Google contains the MAC address
%     \rowcolor{lightgray!15}
%     Apple~\cite{appleprivacy} 
%     & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \Circle\\
%     \rowcolor{lightgray!15}
%     Huawei~\cite{Huaweiprivacy} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \Circle\\
%     Amazon~\cite{} 
%     & \\
    
%     \rowcolor{lightgray!50}
%     \textbf{Academia} &&&&& &&&&&& &&\\
%     \rowcolor{lightgray!15}
%     Yu et al.~\cite{yu2015autoppg} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Wilson et al.~\cite{wilson2016creation} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE  & \CIRCLE
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Harkous et al.~\cite{harkous2018polisis} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE  & \CIRCLE
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Kaur et al.~\cite{kaur2018comprehensive} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE  & \Circle
%     & \CIRCLE & \Circle\\
%     \rowcolor{lightgray!15}
%     Yu et al.~\cite{yu2018enhancing}
%     & \Circle & \Circle & \Circle & \Circle & \Circle
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     & \Circle & \Circle\\
%     \rowcolor{lightgray!15}
%     Zimmeck et al.~\cite{zimmeck2019maps} 
%     & \Circle & \Circle & \Circle & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle
%     & \Circle & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Zhang et al.~\cite{zhang2020does} 
%     & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Sun and Xue~\cite{sun2020quality} 
%     & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle
%     & \CIRCLE & \CIRCLE\\
   
%     \rowcolor{lightgray!15}
%     Li et al.~\cite{li2021developers} 
%     & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     & \CIRCLE & \Circle\\
%     % \rowcolor{lightgray!15}
%     % Only focus on analytics libraries rather than apps
%     % Caputo et al.~\cite{caputo2021you} 
%     % & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
%     % & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     % & \CIRCLE & \Circle\\

%     \rowcolor{lightgray!15}
%     Zimmeck et al.~\cite{zimmeck2021privacyflash} 
%     & \Circle & \Circle & \Circle & \Circle & \Circle 
%     & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \CIRCLE
%     & \Circle & \Circle\\
     
%     \rowcolor{lightgray!15}
%     Xie et al.~\cite{xie2022scrutinizing} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE  & \Circle
%     & \CIRCLE & \CIRCLE\\
%   \hline
% \end{tabular}
% }%
% \end{table*}

==> Tables/ocr_llm_evaluation.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{lccc}
        \hline
        \textbf{Category} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} \\
        \hline
        Name & 0.62 & 0.63 & 0.98 \\
        Birthday  & 1.00 & 1.00 & 1.00 \\
        Address  & 0.47 & 0.50 & 0.89 \\
        Phone  & 0.77 & 0.82 & 0.93 \\
        Email  & 0.67 & 0.97 & 0.68 \\
        Profile  & 0.51 & 0.58 & 0.82 \\
        Contacts  & 0.95 & 0.98 & 0.98 \\
        Location  & 0.87 & 0.89 & 0.97 \\
        Photos  & 0.59 & 0.98 & 0.60 \\
        Voices  & -- & -- & -- \\
        Financial info  & 0.78 & 0.93 & 0.82 \\
        Social media  & 0.50 & 0.58 & 0.78 \\
        \hline
        \textbf{Average} & 0.70 & 0.81 & 0.86 \\
        \hline
    \end{tabular}
    \vspace{-5pt}
    \caption{CDM - Textual GUI components}
    \label{tab:ocr_llm_apr}
\end{table}

==> Tables/segment_success_rate.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|ccc|c}
\toprule
\textbf{Category}    & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{Success Rate}\\
\midrule
Name        & 0.98 & 0.97 & 1.00 & 0.92 \\
Birthday    & 0.94 & 1.00 & 0.94 & 1.00 \\
Address     & 0.48 & 0.82 & 0.50 & 1.00 \\
Phone       & 1.00 & 1.00 & 1.00 & 0.97 \\
Email       & 1.00 & 1.00 & 1.00 & 1.00 \\
Profile     & 0.96 & 0.96 & 1.00 & 0.97 \\
Contacts    & 1.00 & 1.00 & 1.00 & 1.00 \\
Location    & 0.92 & 0.94 & 0.98 & 1.00 \\
Photos      & 0.84 & 0.83 & 1.00 & 1.00 \\
Voices      & 0.85 & 0.33 & 1.00 & 1.00 \\
Financial info   & 1.00 & 1.00 & 1.00 & 1.00 \\
Social media& 1.00 & 1.00 & 1.00 & 1.00 \\
\midrule
\textbf{Average} & 0.92 & 0.94 & 0.98 & 0.99  \\
\bottomrule
\end{tabular}
\caption{Performance of the Segments Extraction Module on the benchmark dataset.}
\label{tab_segment_extraction}
\end{table}

==> Tables/total_detection_results.tex <==
\begin{table}[h]
\centering
\caption{Performance of Overall Context Identification.}
\label{tab_success_rates}
\vspace{-5pt}
\begin{tabular}{lc}
\toprule
\textbf{GUI category} & \textbf{average Context Coverage per screenshot} \\
\midrule
Text     & 87.53\% \\
Icon     & 40.60\% \\
\midrule
\textbf{Overall}  & 83.59\% \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\end{table}




% \begin{table}[h!]
% \centering
% \begin{tabular}{@{}lcc|cc@{}}
% \toprule
%                            & \multicolumn{2}{c}{\textbf{Without Classification}} & \multicolumn{2}{c}{\textbf{With Classification}} \\ \cmidrule(lr){2-3} \cmidrule(l){4-5} 
% \textbf{}                 & \textbf{Precision}          & \textbf{Recall}          & \textbf{Precision}         & \textbf{Recall}          \\ \midrule
% \textbf{Overall}          &              0.1101               &           0.8225               &       0.4977                     &           0.6605               \\
% \textbf{Text}             &              0.1544               &            0.8646              &           0.1933                 &                0.9109          \\
% \textbf{Icon}             &             0.0913                &            0.7211              &           0.2595                 &              0.3579            \\ \bottomrule
% \end{tabular}
% \caption{Precision and recall for detection}
% \label{tab:detection_results}
% \end{table}
